Where's My Head? Definition, Dataset and Models for Numeric Fused-Heads Identification and Resolution

We provide the first computational treatment of fused-heads constructions (FH), focusing on the numeric fused-heads (NFH). FHs constructions are noun phrases (NPs) in which the head noun is missing and is said to be `fused' with its dependent modifier. This missing information is implicit and is important for sentence understanding. The missing references are easily filled in by humans but pose a challenge for computational models. We formulate the handling of FH as a two stages process: identification of the FH construction and resolution of the missing head. We explore the NFH phenomena in large corpora of English text and create (1) a dataset and a highly accurate method for NFH identification; (2) a 10k examples (1M tokens) crowd-sourced dataset of NFH resolution; and (3) a neural baseline for the NFH resolution task. We release our code and dataset, in hope to foster further research into this challenging problem.

==> settings/forest_setup.tex <==
\usepackage{forest}

\makeatletter

\@ifpackagelater{forest}{2016/01/01}
{\useforestlibrary{linguistics}}
{}

\@ifpackagelater{forest}{2016/01/01}
{\newcommand{\forestPreamble}{default preamble}} % version >=2 of forest
  {\newcommand{\forestPreamble}{.style}} % version <=1 of forest

\makeatother
  
\forestset{
  \forestPreamble ={
	% % .style={ % version <=1 of forest
	% default preamble={ % version >=2 of forest    
		for tree={
			parent anchor=south, 
			child anchor=north,
			% align=center,			% bad: adds space below label
			fit=rectangle,
			base=top,				% vertical orientation of nodes
			% inner sep=3,			% necesssary?
			begin draw/.code={\begin{tikzpicture}[baseline=(current bounding box.center)]},
			}},
    sn edges/.style={for tree={parent anchor=south, child anchor=north}},
    red subtree/.style={for tree={text=red},for descendants={edge=red}},
    black subtree/.style={for tree={text=black},for descendants={edge=black}},
    gray subtree/.style={for tree={text=gray},for descendants={edge=gray}},
    vcenter/.style={begin draw/.code={\begin{tikzpicture}[baseline=(current bounding box.center)]}},
      empty nodes/.style={	% from the forest manual
        for tree={
          % calign=fixed edge angles,
          yshift=1ex},
        delay={where content={}{shape=coordinate,for parent={for children={anchor=north}}}{}}},
      derivation tree/.style={.style={
          for tree={parent anchor={},child anchor={},font=\ttfamily}}},
      dt label/.style 2 args={
        edge label={node[midway,font=\ttfamily\scriptsize, #1]{#2}},},
    }

   

    

==> settings/pdflatex_setup.tex <==
%% Font & Encoding
\usepackage{libertine}
\usepackage[libertine]{newtxmath}
\usepackage[scaled=0.8]{beramono}  % for monospaced font
\usepackage{microtype}		% micro-typographic aspects of the fonts
\usepackage[T1]{fontenc}	% special fonts, e.g. for German umlaute
%% incompabtible with Biblatex
% \usepackage{ucs}
% \usepackage[utf8x]{inputenc}
%% compatible with Biblatex
\usepackage[utf8]{inputenc}



%% Language
%\usepackage[german]{babel}
%\usepackage{german}
\usepackage[english]{babel}


 

==> settings/tikz_setup.tex <==
%%%%%%%%%%%%%%%%%%%%%%
%   TIKZ SETTINGS    % 
%%%%%%%%%%%%%%%%%%%%%%

\usepackage{tikz}
\input{packages/tikz-qtree-bugfix}

\tikzset{every tree node/.style={align=center,anchor=north}}	% to allow linebreaks
\usetikzlibrary{calc} % for positioning arrows with ($(t.center)-(1,0)$)
\usetikzlibrary{shapes,decorations}
\usetikzlibrary{backgrounds,fit}
\usetikzlibrary{arrows}
\usetikzlibrary{matrix}
\usetikzlibrary{positioning}
\usetikzlibrary{automata}
\usetikzlibrary{tikzmark}

% Define box and box title style (see http://www.texample.net/tikz/examples/boxes-with-text-and-math/)
\tikzstyle{mybox} = [draw=gray, very thick,
    rectangle, rounded corners, inner sep=10pt, inner ysep=17pt,yshift=3pt]
\tikzstyle{fancytitle} =[draw=gray, very thick, fill=white,
    rectangle, rounded corners, inner sep=5pt, inner ysep=5pt]
\tikzstyle{mydouble} = [double distance=1pt]
    
\tikzset{
    %Define standard arrow tip
    >=stealth',
    %Define style for boxes
    box/.style={
           rectangle,
           rounded corners,
           draw=black, very thick,
           text width=10em,
           minimum height=2em,
           text centered},
    % Define arrow style
    arrow/.style={
           ->,
           thick,
           	shorten <=2pt,
           shorten >=2pt,}
}

\newcommand\centertikz[1]{\tikz[baseline=(current bounding box.center)]{#1}}
\newcommand\tikzcenter{baseline=(current bounding box.center)}
\newcommand\tikztop{baseline=(current bounding box.north)}

\newcommand\tikztreeset[1]{\matrix [matrix of nodes,left delimiter=\{,right delimiter=\}](set){#1};}

==> tables/num-fh-rules.tex <==
\begin{sidewaystable}
% \begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lll}
Fused-Head Type	 		& Rule 	& Example \\ \hline
Conjunction I	 		& $w_{i-1} = \mlq or \mrq \wedge (w_{i+1}.pos \neq NOUN \wedge w_{i+1}.head.pos \neq NOUN$) & Maybe I can teach the kid a thing \textit{or \textbf{two}}. \\
Conjunction II 	 		& $w_{i+1} = \mlq or \mrq$ & \textbf{eight} or nine clubs \\
Particle 				& $w_{i+1} = \mlq 's \mrq \wedge w_{i-1}.pos \neq NOUN \wedge w_{i-1} \neq \mlq \$ \mrq $ & everyone here lives to \textit{their \textbf{90}'s} \\
Time sign 				& $w_{i+1} \in \{a.m, a.m., p.m, p.m.\}$ & \textit{\textbf{Eight} a.m.} you walk the baby. \\
Height					& $w_{i+1} = \mlq ' \mrq \wedge w_{i,i+2} \in [0-9]$ & In my head I'm \textbf{\textit{6'4}}, 190 pound \\
``... the \textbf{one} who ..." 	& $w_{i}.pos = NUM \wedge w_{i-1}=\mlq the \mrq \wedge w_{i+1}=\mlq who \mrq $ & I'M NOT \textit{THE \textbf{ONE}} WHO WATCHES WRESTLING\\
``... \textbf{one} of ..." 		& $w_{i}.pos = NUM \wedge w_{i+1} = \mlq of \mrq$ & Is this little talk \textit{\textbf{one} of} 'em? \\
``... you \textbf{two} ..." 		& $w_{i-1}= \mlq you \mrq \wedge w_{i}=\mlq two \mrq $ & You \textbf{two} are going into her school \\
``... no \textbf{one} ..." 		& $w_{i-1} = \mlq no \mrq \wedge w_{i} = \mlq one \mrq$ & There's \textit{no \textbf{one}} new

\end{tabular}
}
\caption{Common fused-head phenomena which we observed from the data. A large portion of those weren't caught by the constituency parser, and thus appeared as negative examples. We retrieved those rules and added them to the positive examples. The Detection column describes the rule for detecting those cases, and the Example column shows filtered cases from the dataset, which were excluded from the negative examples (and are actually fused-heads). $w_i$ stands for the numbers' span and $w_{i+1},w_{i-1}$ represent the token after / before the number respectively. $.pos$ refers to the token POS tag. All equalities checks are done on lower-cased tokens. Bold tokens are the numbers which actually are fused-heads and the italic span indicates the rule for filtering those cases out. The two last rules (you two... and no one...) are on those specific numbers and doesn't hold on general numbers, as tested on a development set}
\label{tab:num-fh-rules}
% \end{table}
\end{sidewaystable}
